RF Helicon Plasma Thruster for an Atmosphere-Breathing Electric Propulsion System (ABEP)

This dissertation focuses on Atmosphere-Breathing Electric Propulsion (ABEP) for propellant-less continuous orbiting in very low Earth orbits (VLEO) and very low Mars orbits (VLMO). ABEP utilizes an intake to collect atmospheric particles as propellant for an electric thruster, offsetting aerodynamic drag. An analytical system-level analysis assesses collectible mass flow, drag, and power requirements, using GOCE as a case study. Three intake designs are developed based on gas-surface interactions. Two diffuse-reflection designs yield collection efficiencies $\eta_c < 0.5$, while a specular-reflection design achieves $\eta_c < 0.95$. The specular intake demonstrates superior robustness against flow misalignment, maintaining high efficiency at large angles. The proposed ABEP thruster features a contactless, neutralizer-free design using a helicon plasma discharge, preventing erosion from aggressive species like atomic oxygen. Numerical simulations via the HELIC code determined key design parameters (frequency, magnetic field, plasma density), leading to the implementation of a resonant birdcage antenna with high electrical efficiency. The thruster was manufactured and experimentally validated using Ar, N_2, and O_2. Tests demonstrated successful ignition and operation across relevant mass flows with low power consumption ($P_f < 60$ W). Additionally, a B-dot probe was developed to detect helicon waves in the plasma plume. Ultimately, this work delivers verified intake designs and a novel contactless plasma thruster with high electrical efficiency (>99% in vacuum). Both components represent promising technologies for near-future ABEP applications. Future development outlooks, diagnostics, and spacecraft configurations are also discussed.

==> abstractDE.tex <==
Diese Dissertation befasst sich mit der Entwicklung Atmosphärenatmendes, elektrischen Raumfahrtantriebssystems (ABEP), das einen treibstofflosen kontinuierlichen Betrieb in sehr niedrigen Erdumlaufbahnen (VLEO) ermöglichen kann. Das Antriebsystem verwendet einen Einlass vor dem Raumfahrzeug, um die Restatmosphäre zu sammeln und sie an ein elektrisches Triebwerk als Treibstoff zu liefern, um schließlich die Ursache des aerodynamischen Widerstands als Quelle des Schubs zu nutzen. 

In einer Literaturübersicht wird der Stand der Technik von ABEP dargestellt und die wichtigsten Leistungsparameter werden hervorgehoben. Die Anwendung von ABEP in VLEO wird untersucht, indem analytische Gleichungen auf der Basis von Atmosphärenmodellen und Einlasswirkungsgraden angewendet werden, die auf den Ergebnissen dieser Arbeit und den verfügbaren Triebwerkswirkungsgraden nach dem Stand der Technik basieren. Diese Analyse leitet den sammelbaren Treibstofffluss, den aerodynamischen Widerstand und die zur vollständigen Kompensation des Widerstands erforderliche Leistung ab.  Der Fall von GOCE unter Verwendung eines ABEP-Systems wird vorgestellt, ebenso wie seine Anwendung im sehr niedrigen Mars-Orbit (VLMO).

Der Einlass und das Triebwerk werden in dieser Dissertation untersucht und entworfen. 

Es werden drei ABEP-Einlassdesigns vorgestellt, die auf den Eigenschaften der\\ Gas-Oberflächen-Wechselwirkung basieren. Zwei basieren auf vollständig diffusen Reflexionen, die einen Einlasswirkungsgrad $\eta_{c,max}<0.5$ liefern, und eines basiert auf vollständig spiegelnden Reflexionen, welches signifikant höhere Einlasswirkungsgrade ermöglicht\\ ($\eta_{c,max}<0.95$). Ihre jeweilige Empfindlichkeit gegenüber Fehlausrichtung mit der Strömung wird ebenfalls analysiert, wobei das spiegelnde Design im Vergleich zum diffusen robuster ist, da es auch bei großen Winkeln relativ hohe $\eta_c$ beibehält. 

Das ABEP-Triebwerk basiert auf einer kontaktlosen Technologie: Es gibt keine Komponente, die in direktem Kontakt mit dem Plasma steht, und es wird ein quasi-neutraler Plasmastrahl erzeugt. Dies ermöglicht den Betrieb mit mehreren Treibstoffarten  insbesondere auch mit atomarem Sauerstoff als einer der Hauptkomponenten der Restatmosphäre im VLEO, und Dichten und erfordert keinen Neutralisator. Das Triebwerk basiert auf Helikon-Plasmaentladungen, um eine höhere Effizienz im Vergleich zu induktiven Entladungen zu erreichen.	

Eine numerische Untersuchung zur Bestimmung der grundlegenden Designparameter des Triebwerks, wie Eingangsfrequenz, Antennedesign, Plasmadichte und erforderliches Magnetfeld, wird mit dem HELIC-Code durchgeführt. Die Analyse führte zur Anwendung der Birdcage-Antenne, die simuliert, aufgebaut und experimentell verifiziert wurde. Sie arbeitet in Resonanz und ist Impedanz-angepasst, was zu einem hohen elektrischen Wirkungsgrad führt. Das Triebwerk wurde integriert und an \ce{Ar}, \ce{N2} und \ce{O2} getestet. Die erfolgreichen Tests zeigen eine niedrige Leistungsaufnahme $P_f<\SI{60}{\watt}$ und die Fähigkeit der Zündung und des Betriebs für zahlreiche Treibstoffe unter Variation der Massenströme, die innerhalb des erwarteten ABEP-Bereichs liegen. Darüber hinaus wird eine B-Dot-Sonde entworfen und aufgebaut, die darauf abzielt, Helikon-Wellen innerhalb des Plasmastrahls zu detektieren.

Zusammenfassend wurde in dieser Dissertation die größte Herausforderung zur kontinuierlichen Überwindung des Luftwiderstands in niedrigen Umlaufbahnen untersucht und eine spezifische ABEP-Lösung vorgeschlagen. Dies führte zu drei effizienten Einlassdesigns, die auf verifizierten Partikelsimulationen basieren, und zu einem neuartigen kontaktlosen, Helikon-basierten Plasmatriebwerk. Letzteres wurde verifiziert, gebaut und getestet. Es liefert einen hohen elektrischen Wirkungsgrad, $>99\%$, kann mit atmosphärischem Treibstoff betrieben werden und benötigt sehr geringe Eingangsleistungen, $P_f\sim\SI{60}{\watt}$. Daher sind sowohl Einlass als auch Triebwerk\\ vielversprechende Technologien für eine baldige reale Weltraumanwendung des ABEP-Systems.

Darüber hinaus werden Ausblicke und Verbesserungen für die ABEP-Entwicklung und die erforderliche Diagnostik vorgestellt, einschließlich potenzieller ABEP-basierter\\ Raumfahrzeugkonfigurationen für die langfristige Entwicklung des ABEP-Systems.

==> nomenclature.tex <==
\begin{tabular}{lp{0.6\textwidth}}
\textbf{ABEP} & Atmosphere-Breathing Electric Propulsion\\
\textbf{ADCS} & Attitude Determination and Control System\\
\textbf{AC} & Direct Current\\
\textbf{AO} & Atomic Oxygen\\
\textbf{AR} & Anti-Rotating\\
\textbf{CFDL} & Current Free Double Layer\\
\textbf{CR} & Co-Rotating\\
\textbf{DAQ} & Data Acquisition\\
\textbf{DC} & Direct Current\\
\textbf{DSMC} & Direct Simulation Monte Carlo\\
\textbf{ECR} & Electron Cyclotron Resonance\\
\textbf{EFD} & Enhanced Funnel Design\\
\textbf{EM} & Electromagnetic\\
\textbf{EP} & Electric Propulsion\\
\textbf{FDTD} & Finite-Difference Time-Domain\\
\textbf{FMF} & Free Molecular Flow\\
\textbf{GIT} & Gridded Ion Thruster\\
\textbf{GSI} & Gas Surface Interactions\\
\textbf{HET} & Hall-Effect Thruster\\
\textbf{HHT} & Helicon Hall-Effect Thruster\\
\textbf{HOPH} & Highly Oriented Pyrolytic Graphite\\
\textbf{HPT} & Helicon Plasma Thruster\\
\textbf{ICP} & Inductively Coupled Plasma\\
\textbf{ICR} & Ion Cyclotron Resonance\\
\textbf{IGP} & Inductively-heated Plasma Generator\\
\textbf{IPT} & RF Helicon-based Plasma Thruster\\
\textbf{MCD} & Mars Climate Database\\
\textbf{MFC} & Mass Flow Controller\\
\textbf{PCB} & Printed Circuit Board\\
\textbf{PPU} & Power Processing Unit\\
\textbf{RAID} & Resonant Antenna Ion Device\\
\textbf{RF} & Radio Frequency\\
\textbf{RIT} & Radio Frequency Ion Thruster\\
\textbf{SC} & Spacecraft\\
\textbf{SSO} & Sun-Synchronous Orbit\\
\textbf{TG} & Trivelpiece-Gould\\
\textbf{VF} & Velocity Factor\\
\textbf{VLEO} & Very Low Earth Orbit\\
\textbf{VLMO} & Very Low Mars Orbit\\
\textbf{VLO} & Very Low Orbit\\
\end{tabular}



==> symbols.tex <==
$\alpha=$ Accommodation Coefficient, -
$A_f=$ Frontal Area m2
$A_{in}=$ Intake Area m2
$A_{out}=$ Outlet Area m2
$A_{SA}=$ Solar Array Area m2
$Ap=$ Geomagnetic Index
$\beta=$ Flow Angle to Intake Symmetry Axis $\degree$
$\vec{B}$ Vector Magnetic Field T
$c=$ Speed of Light m/s
$c_e=$ Exhaust Velocity m/s
$C_D=$ Drag Coefficient
$c_s=$ Velocity of Sound Waves in Plasma m/s
$d=$ Diameter, m
$D=$ Aerodynamic Drag mN
$\eta_c=$ Collection Efficiency 
$\eta_T=$ Thruster Efficiency
$\epsilon_0$ Permittivity of Free Space F/m 
$e$ Electron Charge C
$\vec{E}$ Vector Electric Field V/m
$E_i=$ Energy of the Incoming Molecule, J
$E_r=$ Energy of the Re-emitted Molecule, J
$E_w=$ Energy of the Re-emitted Molecule if Equalized to Wall Temperature, J
$F10.7_{avg}=$ Average Solar Radio Flux at $\lambda=\SI{10.7}{\centi\meter}$, $sfu$
$F_f$ Filling Factor -
$\gamma$ Adiabatic Index -
$h=$ altitude km
$f=$ Frequency Hz, MHz
$I_{sp}=$ Specific Impulse s
$k=$ Wave Number rad/m
$k_B=$ Boltzmann Constant
$\lambda=$ Wavelength m
$\lambda_D$ Debye Length m
$L=$ Length m
$\mu_0$ Permeability of Vacuum H/m
$m=$ Mass kg
$m=$ Helicon Wave Mode Number
$M=$ Ion Mass kg
$\dot{m}_{thr}=$ Mass Flow Reaching the Thruster mg/s
$n=$ Number Density 1/m3
$n_e$ Electron Density 1/m3
$n_i$ Ion Density 1/m3
$N_{int}$ Number of Intakes
$N_{ducts}$ Number of Ducts
$\dot{N}_{in}=$ Incoming Particle Flux 1/s
$\dot{N}_{out}=$ Outgoing Particle Flux 1/s
$\dot{N}_{thr}=$ Particle Flux Reaching the Thruster 1/s

$p=$ Pressure Pa
$p_$ Electron Pressure Pa
$p_{in}=$ Input Thruster Pressure Pa
$p_{ch}=$ Chamber Pressure Pa
$P=$ Power W
$P_{ABEP}$ ABEP Power W
$P_{in}=$ Power Input W
$P_{jet}=$ Jet Power W
$P_{RF}=$ Radio Frequency Power W
$\rho=$ Mass Density kg/m3
$q=$ Elementary Charge C
$r_L$ Larmor Radius m
$R=$ Radius m
$R_C=$ Circuit Resistance Ohm
$R_P=$ Plasma Resistance Ohm
$S=$ Molecular Speed Ratio
$\Theta$ Transmission Probability
$T =$ Thrust mN 
$T_e=$ Electron Temperature K
$T/P=$ Thrust-to-Power ratio mN/kW
$u=$ Velocity m/s
$v=$ Orbital Velocity m/s
$v=$ Alfvén Velocity m/s
$v_{\phi}=$ Phase Velocity m/s
$v_g$ Group Velocity m/s
$v_s$ Speed of Sound in Plasma m/s
$v_{th}$ Thermal Velocity 
$\omega$ Angular Frequency rad/s
$\omega_c$ Electron Cyclotron Frequency rad/s
$\omega_h$ Hybrid Frequency rad/s
$\omega_{Helicon}$ Helicon Wave Frequency rad/s
$\omega_l$ Lower Hybrid Frequency rad/s
$\omega_L,R$ Plasma Cutoff Frequency rad/s
$\omega_p$ Plasma Frequency rad/s
$\Omega_c$ Ion Cyclotron Frequency rad/s
$W=$ width m
$X=$ Dimensionless Inflow Parameter -
$Z=$ 






==> thruster.tex <==
The thruster is the main focus on this dissertation. The basis is the development of a contact-less RF-based electric thruster, so to remove any issue of performance degradation over time due to operation with aggressive species such as atomic oxygen \ce{O} as propellant. The plasma exhaust is expected to be quasi-neutral, therefore removing the need of a neutralizer. Furthermore, such contact-less devices are able to cope with variations of propellant density and composition by changing the input power. The development of the RF helicon-based inductive plasma thruster (IPT) started from a long heritage at IRS on inductively coupled plasma sources. 
The IPT concept is of an RF-fed antenna that surrounds the discharge channel in which the propellant is injected. The RF-fed antenna launches electromagnetic waves within the discharge channel exciting the propellant particles: it ionizes them and, in combination with the external magnetic field, accelerates them through the exhaust producing thrust, see Fig.~\ref{fig:IPT}.  The contact-less nature of the IPT does not only remove any erosion issue, but also enhances the propellant flexibility, making it able to cope with basically any propellant also at variable amount and composition. The most efficient RF discharge is the helicon wave-based discharge. Such high efficiency is necessary to minimize power consumption as well as to achieve electromagnetic acceleration necessary to produce high enough exhaust velocities. Therefore the IPT design can cope with the following challenges:
\begin{itemize}
	\item RF contact-less design:
	\begin{itemize}
		\item minimizes erosion issues;
		\item copes with propellant composition and density variation;
		\item copes with any propellant;
	\end{itemize}
	\item Quasi-neutral plasma plume $\Rightarrow$ Neutralizer not required.
\end{itemize}
The conceptual schematics of the IPT, including the respective RF generator, matching network, and solenoid DC power supply, is shown within Fig.~\ref{fig:IPT}.
\begin{figure}[h]
	\centering
	\includegraphics[width=15cm]{bilder/IPT/IPT_concept.png}
	\caption{RF Helicon-based Inductive Plasma Thruster (IPT) Concept.}
	\label{fig:IPT}
\end{figure}

The plasma thruster design, as well as its physics, are described into detail in Chapter~\ref{ch:plasma} and~\ref{ch:IPT}.
